Logistic-Normal Likelihoods for Heteroscedastic Label Noise

A natural way of estimating heteroscedastic label noise in regression is to model the observed (potentially noisy) target as a sample from a normal distribution, whose parameters can be learned by minimizing the negative log-likelihood. This formulation has desirable loss attenuation properties, as it reduces the contribution of high-error examples. Intuitively, this behavior can improve robustness against label noise by reducing overfitting. We propose an extension of this simple and probabilistic approach to classification that has the same desirable loss attenuation properties. Furthermore, we discuss and address some practical challenges of this extension. We evaluate the effectiveness of the method by measuring its robustness against label noise in classification. We perform enlightening experiments exploring the inner workings of the method, including sensitivity to hyperparameters, ablation studies, and other insightful analyses.

==> 7_tables_syntheticnoise.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t!]
\tabcolsep=0.15cm 
\caption{\label{tab:synthetic} \textbf{Synthetic Noise on MNIST, CIFAR-10 and CIFAR-100.} We implement our method and all baselines in the same shared code based and do a search for the best hyperparameters on a noisy validation set for all methods. We report the mean and standard deviation of the test accuracy from five runs with different random seeds. Results in bold correspond to the methods with no statistically significant difference to the method with the highest mean. Our method~(LN) shows strong performance compared to baselines, especially on the  predictable asymmetric noise, and the challenging CIFAR-100 dataset.  
}
\begin{center}
\begin{tabular}{ m{1em} l c c c c c c c c c@{}} 
 \toprule
 \multirow{2}{0em}{} & \multirow{2}{4em}{Method} & No Noise & \multicolumn{4}{c}{Symmetric Noise Rate} & \multicolumn{4}{c}{Asymmetric Noise Rate}  \\ \cmidrule(lr){3-3}\cmidrule(lr){4-7} \cmidrule(lr){8-11}
 & & 0\% & 20\% & 40\% & 60\% & 80\% & 10\% & 20\% & 30\% & 40\% \\
 \midrule
 \multirow{8}{2em}{\rotatebox[origin=c]{90}{MNIST}}
& CE & 99.27 $\pm$ 0.07 &  88.41 $\pm$ 0.34 &  70.67 $\pm$ 1.30 &  51.04 $\pm$ 1.19 &  29.53 $\pm$ 1.08 & 96.64 $\pm$ 0.32 &  91.09 $\pm$ 0.79 &  86.31 $\pm$ 1.25 &  80.31 $\pm$ 1.81 \\
& Bi-tempered & 99.22 $\pm$ 0.05 &  97.79 $\pm$ 0.69 &  97.78 $\pm$ 0.29 &  83.26 $\pm$ 1.50 &  53.76 $\pm$ 2.58  & 96.52 $\pm$ 0.28 &  97.33 $\pm$ 0.16 &  96.67 $\pm$ 0.51 &  86.45 $\pm$ 1.79 \\
& GCE & 99.22 $\pm$ 0.06 &  \textbf{98.85} $\pm$ \textbf{0.18} &  \textbf{98.60} $\pm$ \textbf{0.11} &  \textbf{97.45} $\pm$ \textbf{0.31} &  \textbf{92.60} $\pm$ \textbf{0.61} & 98.98 $\pm$ 0.12 &  98.52 $\pm$ 0.31 &  86.36 $\pm$ 0.86 &  79.81 $\pm$ 1.46 \\
& NAN & 98.44 $\pm$ 0.24 &  97.51 $\pm$ 0.37 &  90.03 $\pm$ 0.95 &  74.00 $\pm$ 2.92 &  46.25 $\pm$ 2.03 & 97.04 $\pm$ 1.23 &  96.46 $\pm$ 2.23 &  95.43 $\pm$ 1.09 &  88.95 $\pm$ 1.63 \\
& Forward & 99.27 $\pm$ 0.03 &  87.46 $\pm$ 0.70 &  69.96 $\pm$ 2.10 &  50.43 $\pm$ 1.43 &  30.01 $\pm$ 0.60 & 96.51 $\pm$ 0.55 &  91.95 $\pm$ 0.40 &  86.31 $\pm$ 0.43 &  80.97 $\pm$ 1.23 \\
& Het & 99.28 $\pm$ 0.05 &  87.09 $\pm$ 0.70 &  70.30 $\pm$ 1.10 &  50.57 $\pm$ 1.02 &  29.88 $\pm$ 0.88 & 96.45 $\pm$ 0.35 &  91.12 $\pm$ 1.29 &  86.35 $\pm$ 0.62 &  80.04 $\pm$ 0.87 \\
& Het-$\tau$ & 99.25 $\pm$ 0.07 &  88.10 $\pm$ 0.70 &  70.19 $\pm$ 1.58 &  51.95 $\pm$ 1.13 &  31.81 $\pm$ 0.86 & 96.07 $\pm$ 0.45 &  91.13 $\pm$ 1.25 &  85.95 $\pm$ 0.69 &  81.37 $\pm$ 1.14\\
& Het-$\tau$-$\bm{\Sigma}_{\textbf{full}}$ & \textbf{99.25} $\pm$ \textbf{0.15} &  89.16 $\pm$ 0.44 &  70.34 $\pm$ 1.20 &  50.89 $\pm$ 1.79 &  30.54 $\pm$ 0.69 & 96.74 $\pm$ 0.19 &  91.06 $\pm$ 0.24 &  86.25 $\pm$ 0.88 &  79.93 $\pm$ 0.44 \\
& LN & \textbf{99.38} $\pm$ \textbf{0.06} &  \textbf{98.53} $\pm$ \textbf{0.27} &  97.21 $\pm$ 0.38 &  90.93 $\pm$ 2.29 &  60.15 $\pm$ 5.01 & \textbf{99.24} $\pm$ \textbf{0.06} &  \textbf{99.19} $\pm$ \textbf{0.10} &  \textbf{99.01} $\pm$ \textbf{0.19} &  \textbf{96.54} $\pm$ \textbf{1.20} \\
\midrule
\multirow{8}{2em}{\rotatebox[origin=c]{90}{CIFAR-10}} 
& CE & \textbf{90.67} $\pm$ \textbf{0.80} &  73.54 $\pm$ 1.01 &  56.56 $\pm$ 1.44 &  39.44 $\pm$ 1.87 &  21.91 $\pm$ 1.35 & 85.56 $\pm$ 0.53 &  81.35 $\pm$ 1.26 &  76.01 $\pm$ 2.67 &  71.89 $\pm$ 1.67  \\
& Bi-tempered & 89.89 $\pm$ 0.50 &  85.68 $\pm$ 0.38 &  75.70 $\pm$ 2.16 &  51.55 $\pm$ 4.66 &  32.18 $\pm$ 2.31 & 85.49 $\pm$ 0.75 &  81.79 $\pm$ 1.40 &  78.74 $\pm$ 1.66 &  71.60 $\pm$ 1.37 \\
& GCE & \textbf{90.83} $\pm$ \textbf{0.44} &  \textbf{87.55} $\pm$ \textbf{0.41} &  \textbf{84.72} $\pm$ \textbf{0.82} &  \textbf{79.25} $\pm$ \textbf{0.93} &  \textbf{64.28} $\pm$ \textbf{1.42} & \textbf{88.02} $\pm$ \textbf{0.20} &  85.68 $\pm$ 0.69 &  83.97 $\pm$ 0.52 &  72.90 $\pm$ 1.61 \\
& NAN & 89.61 $\pm$ 0.93 &  83.86 $\pm$ 1.03 &  79.80 $\pm$ 0.59 &  73.58 $\pm$ 0.41 &  61.06 $\pm$ 1.84 & 86.55 $\pm$ 0.72 &  84.32 $\pm$ 1.05 &  76.79 $\pm$ 2.28 &  72.90 $\pm$ 1.92 \\
& Forward & \textbf{90.69} $\pm$ \textbf{0.38} &  74.39 $\pm$ 1.49 &  59.60 $\pm$ 1.40 &  40.06 $\pm$ 2.16 &  23.80 $\pm$ 1.00 & 86.17 $\pm$ 0.65 &  82.10 $\pm$ 1.09 &  77.02 $\pm$ 2.38 &  72.77 $\pm$ 1.43 \\
& Het & \textbf{90.41} $\pm$ \textbf{0.69} &  74.67 $\pm$ 1.06 &  58.53 $\pm$ 1.96 &  39.51 $\pm$ 2.53 &  24.18 $\pm$ 0.67 & 86.26 $\pm$ 0.40 &  81.72 $\pm$ 1.65 &  76.97 $\pm$ 1.17 &  72.88 $\pm$ 1.53 \\
& Het-$\tau$ & \textbf{91.18} $\pm$ \textbf{0.41} &  76.90 $\pm$ 1.79 &  63.55 $\pm$ 2.27 &  44.73 $\pm$ 1.67 &  26.36 $\pm$ 1.58 & 86.02 $\pm$ 0.61 &  81.40 $\pm$ 0.96 &  77.41 $\pm$ 2.53 &  72.53 $\pm$ 1.83 \\
& Het-$\tau$-$\bm{\Sigma}_{\textbf{full}}$ & \textbf{90.82} $\pm$ \textbf{0.42} &  77.16 $\pm$ 0.94 &  62.85 $\pm$ 1.88 &  44.20 $\pm$ 3.05 &  25.11 $\pm$ 2.20 & 86.41 $\pm$ 0.55 &  81.55 $\pm$ 0.80 &  77.05 $\pm$ 0.33 &  72.69 $\pm$ 0.89 \\
& LN & 90.17 $\pm$ 0.55 &  86.13 $\pm$ 1.03 &  81.37 $\pm$ 1.97 &  76.08 $\pm$ 0.63 &  \textbf{63.58} $\pm$ \textbf{1.76} & \textbf{88.25} $\pm$ \textbf{0.53} &  \textbf{87.64} $\pm$ \textbf{0.78} &  \textbf{86.91} $\pm$ \textbf{1.03} &  \textbf{82.18} $\pm$ \textbf{1.30} \\
\midrule
\multirow{8}{2em}{\rotatebox[origin=c]{90}{CIFAR-100}} 
& CE & \textbf{64.87} $\pm$ \textbf{0.88} &  47.39 $\pm$ 0.43 &  33.62 $\pm$ 0.79 &  20.04 $\pm$ 0.58 &  7.38 $\pm$ 0.12 & 57.52 $\pm$ 0.65 &  50.98 $\pm$ 0.88 &  44.04 $\pm$ 0.73 &  36.95 $\pm$ 0.58 \\
& Bi-tempered & \textbf{64.75} $\pm$ \textbf{0.15} &  58.32 $\pm$ 0.69 &  49.05 $\pm$ 0.47 &  29.51 $\pm$ 0.67 &  10.53 $\pm$ 0.67 & 60.17 $\pm$ 0.79 &  53.04 $\pm$ 0.94 &  44.96 $\pm$ 0.52 &  36.95 $\pm$ 0.90 \\
& GCE & \textbf{64.33} $\pm$ \textbf{0.83} &  \textbf{61.67} $\pm$ \textbf{0.67} &  \textbf{53.96} $\pm$ \textbf{1.40} &  42.85 $\pm$ 0.79 &  10.77 $\pm$ 0.28 & \textbf{62.34} $\pm$ \textbf{0.67} &  59.63 $\pm$ 1.28 &  49.21 $\pm$ 0.53 &  36.78 $\pm$ 0.50  \\
& NAN & \textbf{64.25} $\pm$ \textbf{0.64} &  56.93 $\pm$ 0.77 &  50.03 $\pm$ 0.62 &  40.45 $\pm$ 0.41 &  \textbf{24.00} $\pm$ \textbf{0.59} & 60.55 $\pm$ 0.71 &  56.40 $\pm$ 1.07 &  52.78 $\pm$ 0.85 &  40.59 $\pm$ 0.84 \\
& Forward & \textbf{64.33} $\pm$ \textbf{0.73} &  47.90 $\pm$ 0.93 &  32.28 $\pm$ 1.10 &  20.00 $\pm$ 0.75 &  7.64 $\pm$ 0.28 & 58.46 $\pm$ 0.53 &  50.82 $\pm$ 0.57 &  43.87 $\pm$ 0.47 &  37.02 $\pm$ 0.72 \\
& Het & \textbf{64.48} $\pm$ \textbf{0.31} &  48.40 $\pm$ 1.32 &  34.26 $\pm$ 0.37 &  20.33 $\pm$ 0.31 &  7.66 $\pm$ 0.38 & 58.18 $\pm$ 0.31 &  51.44 $\pm$ 1.15 &  45.09 $\pm$ 0.40 &  37.43 $\pm$ 0.66 \\
& Het-$\tau$ & \textbf{64.20} $\pm$ \textbf{0.37} &  54.17 $\pm$ 0.79 &  42.03 $\pm$ 0.84 &  22.33 $\pm$ 0.57 &  7.31 $\pm$ 0.37 & \textbf{62.71} $\pm$ \textbf{0.75} &  59.89 $\pm$ 0.54 &  53.75 $\pm$ 1.08 &  41.14 $\pm$ 0.98 \\
& Het-$\tau$-$\bm{\Sigma}_{\textbf{full}}$ & \textbf{65.18} $\pm$ \textbf{0.90} &  54.83 $\pm$ 0.46 &  41.49 $\pm$ 1.53 &  22.42 $\pm$ 0.95 &  7.77 $\pm$ 0.27 & 61.88 $\pm$ 0.85 &  61.29 $\pm$ 0.46 &  56.44 $\pm$ 0.53 &  45.75 $\pm$ 1.02 \\
& LN & \textbf{64.88} $\pm$ \textbf{0.98} &  \textbf{60.58} $\pm$ \textbf{1.07} &  \textbf{55.55} $\pm$ \textbf{1.30} &  \textbf{46.43} $\pm$ \textbf{1.15} &  \textbf{23.64} $\pm$ \textbf{1.02} & \textbf{63.35} $\pm$ \textbf{0.75} &  \textbf{64.31} $\pm$ \textbf{0.98} &  \textbf{64.07} $\pm$ \textbf{0.77} &  \textbf{61.20} $\pm$ \textbf{1.22} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> 7_tables_syntheticnoise_asym.tex.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t!]
\tabcolsep=0.15cm 
\caption{\label{tab:synthetic-asym} \textbf{Synthetic Noise on MNIST, CIFAR-10 and CIFAR-100.} We implement our method and all baselines in the same shared code based and do a search for the best hyperparameters on a noisy validation set for all methods. We report the mean and standard deviation of the test accuracy from five runs with different random seeds. Results in bold correspond to the methods with no statistically significant difference to the method with the highest mean. Our method~(LN) shows strong performance compared to baselines, especially on the  predictable asymmetric noise, and the challenging CIFAR-100 dataset.  
}
\begin{center}
\begin{tabular}{ m{1em} l c c c c c c c c c@{}} 
 \toprule
 \multirow{2}{0em}{} & \multirow{2}{4em}{Method} & No Noise & \multicolumn{4}{c}{Symmetric Noise Rate} & \multicolumn{4}{c}{Asymmetric Noise Rate}  \\ \cmidrule(lr){3-3}\cmidrule(lr){4-7} \cmidrule(lr){8-11}
 & & 0\% & 20\% & 40\% & 60\% & 80\% & 10\% & 20\% & 30\% & 40\% \\
 \midrule
 \multirow{8}{2em}{\rotatebox[origin=c]{90}{MNIST}}
& CE & 99.27 $\pm$ 0.07 &  88.41 $\pm$ 0.34 &  70.67 $\pm$ 1.30 &  51.04 $\pm$ 1.19 &  29.53 $\pm$ 1.08 & 96.64 $\pm$ 0.32 &  91.09 $\pm$ 0.79 &  86.31 $\pm$ 1.25 &  80.31 $\pm$ 1.81 \\
& Bi-tempered & 99.22 $\pm$ 0.05 &  97.79 $\pm$ 0.69 &  97.78 $\pm$ 0.29 &  83.26 $\pm$ 1.50 &  53.76 $\pm$ 2.58  & 96.52 $\pm$ 0.28 &  97.33 $\pm$ 0.16 &  96.67 $\pm$ 0.51 &  86.45 $\pm$ 1.79 \\
& GCE & 99.22 $\pm$ 0.06 &  \textbf{98.85} $\pm$ \textbf{0.18} &  \textbf{98.60} $\pm$ \textbf{0.11} &  \textbf{97.45} $\pm$ \textbf{0.31} &  \textbf{92.60} $\pm$ \textbf{0.61} & 98.98 $\pm$ 0.12 &  98.52 $\pm$ 0.31 &  86.36 $\pm$ 0.86 &  79.81 $\pm$ 1.46 \\
& NAN & 98.44 $\pm$ 0.24 &  97.51 $\pm$ 0.37 &  90.03 $\pm$ 0.95 &  74.00 $\pm$ 2.92 &  46.25 $\pm$ 2.03 & 97.04 $\pm$ 1.23 &  96.46 $\pm$ 2.23 &  95.43 $\pm$ 1.09 &  88.95 $\pm$ 1.63 \\
& Forward & 99.27 $\pm$ 0.03 &  87.46 $\pm$ 0.70 &  69.96 $\pm$ 2.10 &  50.43 $\pm$ 1.43 &  30.01 $\pm$ 0.60 & 96.51 $\pm$ 0.55 &  91.95 $\pm$ 0.40 &  86.31 $\pm$ 0.43 &  80.97 $\pm$ 1.23 \\
& Het & 99.28 $\pm$ 0.05 &  87.09 $\pm$ 0.70 &  70.30 $\pm$ 1.10 &  50.57 $\pm$ 1.02 &  29.88 $\pm$ 0.88 & 96.45 $\pm$ 0.35 &  91.12 $\pm$ 1.29 &  86.35 $\pm$ 0.62 &  80.04 $\pm$ 0.87 \\
& Het-$\tau$ & 99.25 $\pm$ 0.07 &  88.10 $\pm$ 0.70 &  70.19 $\pm$ 1.58 &  51.95 $\pm$ 1.13 &  31.81 $\pm$ 0.86 & 96.07 $\pm$ 0.45 &  91.13 $\pm$ 1.25 &  85.95 $\pm$ 0.69 &  81.37 $\pm$ 1.14\\
& Het-$\tau$-$\bm{\Sigma}_{\textbf{full}}$ & \textbf{99.25} $\pm$ \textbf{0.15} &  89.16 $\pm$ 0.44 &  70.34 $\pm$ 1.20 &  50.89 $\pm$ 1.79 &  30.54 $\pm$ 0.69 & 96.74 $\pm$ 0.19 &  91.06 $\pm$ 0.24 &  86.25 $\pm$ 0.88 &  79.93 $\pm$ 0.44 \\
& LN & \textbf{99.38} $\pm$ \textbf{0.06} &  \textbf{98.53} $\pm$ \textbf{0.27} &  97.21 $\pm$ 0.38 &  90.93 $\pm$ 2.29 &  60.15 $\pm$ 5.01 & \textbf{99.24} $\pm$ \textbf{0.06} &  \textbf{99.19} $\pm$ \textbf{0.10} &  \textbf{99.01} $\pm$ \textbf{0.19} &  \textbf{96.54} $\pm$ \textbf{1.20} \\
\midrule
\multirow{8}{2em}{\rotatebox[origin=c]{90}{CIFAR-10}} 
& CE & \textbf{90.67} $\pm$ \textbf{0.80} &  73.54 $\pm$ 1.01 &  56.56 $\pm$ 1.44 &  39.44 $\pm$ 1.87 &  21.91 $\pm$ 1.35 & 85.56 $\pm$ 0.53 &  81.35 $\pm$ 1.26 &  76.01 $\pm$ 2.67 &  71.89 $\pm$ 1.67  \\
& Bi-tempered & 89.89 $\pm$ 0.50 &  85.68 $\pm$ 0.38 &  75.70 $\pm$ 2.16 &  51.55 $\pm$ 4.66 &  32.18 $\pm$ 2.31 & 85.49 $\pm$ 0.75 &  81.79 $\pm$ 1.40 &  78.74 $\pm$ 1.66 &  71.60 $\pm$ 1.37 \\
& GCE & \textbf{90.83} $\pm$ \textbf{0.44} &  \textbf{87.55} $\pm$ \textbf{0.41} &  \textbf{84.72} $\pm$ \textbf{0.82} &  \textbf{79.25} $\pm$ \textbf{0.93} &  \textbf{64.28} $\pm$ \textbf{1.42} & \textbf{88.02} $\pm$ \textbf{0.20} &  85.68 $\pm$ 0.69 &  83.97 $\pm$ 0.52 &  72.90 $\pm$ 1.61 \\
& NAN & 89.61 $\pm$ 0.93 &  83.86 $\pm$ 1.03 &  79.80 $\pm$ 0.59 &  73.58 $\pm$ 0.41 &  61.06 $\pm$ 1.84 & 86.55 $\pm$ 0.72 &  84.32 $\pm$ 1.05 &  76.79 $\pm$ 2.28 &  72.90 $\pm$ 1.92 \\
& Forward & \textbf{90.69} $\pm$ \textbf{0.38} &  74.39 $\pm$ 1.49 &  59.60 $\pm$ 1.40 &  40.06 $\pm$ 2.16 &  23.80 $\pm$ 1.00 & 86.17 $\pm$ 0.65 &  82.10 $\pm$ 1.09 &  77.02 $\pm$ 2.38 &  72.77 $\pm$ 1.43 \\
& Het & \textbf{90.41} $\pm$ \textbf{0.69} &  74.67 $\pm$ 1.06 &  58.53 $\pm$ 1.96 &  39.51 $\pm$ 2.53 &  24.18 $\pm$ 0.67 & 86.26 $\pm$ 0.40 &  81.72 $\pm$ 1.65 &  76.97 $\pm$ 1.17 &  72.88 $\pm$ 1.53 \\
& Het-$\tau$ & \textbf{91.18} $\pm$ \textbf{0.41} &  76.90 $\pm$ 1.79 &  63.55 $\pm$ 2.27 &  44.73 $\pm$ 1.67 &  26.36 $\pm$ 1.58 & 86.02 $\pm$ 0.61 &  81.40 $\pm$ 0.96 &  77.41 $\pm$ 2.53 &  72.53 $\pm$ 1.83 \\
& Het-$\tau$-$\bm{\Sigma}_{\textbf{full}}$ & \textbf{90.82} $\pm$ \textbf{0.42} &  77.16 $\pm$ 0.94 &  62.85 $\pm$ 1.88 &  44.20 $\pm$ 3.05 &  25.11 $\pm$ 2.20 & 86.41 $\pm$ 0.55 &  81.55 $\pm$ 0.80 &  77.05 $\pm$ 0.33 &  72.69 $\pm$ 0.89 \\
& LN & 90.17 $\pm$ 0.55 &  86.13 $\pm$ 1.03 &  81.37 $\pm$ 1.97 &  76.08 $\pm$ 0.63 &  \textbf{63.58} $\pm$ \textbf{1.76} & \textbf{88.25} $\pm$ \textbf{0.53} &  \textbf{87.64} $\pm$ \textbf{0.78} &  \textbf{86.91} $\pm$ \textbf{1.03} &  \textbf{82.18} $\pm$ \textbf{1.30} \\
\midrule
\multirow{8}{2em}{\rotatebox[origin=c]{90}{CIFAR-100}} 
& CE & \textbf{64.87} $\pm$ \textbf{0.88} &  47.39 $\pm$ 0.43 &  33.62 $\pm$ 0.79 &  20.04 $\pm$ 0.58 &  7.38 $\pm$ 0.12 & 57.52 $\pm$ 0.65 &  50.98 $\pm$ 0.88 &  44.04 $\pm$ 0.73 &  36.95 $\pm$ 0.58 \\
& Bi-tempered & \textbf{64.75} $\pm$ \textbf{0.15} &  58.32 $\pm$ 0.69 &  49.05 $\pm$ 0.47 &  29.51 $\pm$ 0.67 &  10.53 $\pm$ 0.67 & 60.17 $\pm$ 0.79 &  53.04 $\pm$ 0.94 &  44.96 $\pm$ 0.52 &  36.95 $\pm$ 0.90 \\
& GCE & \textbf{64.33} $\pm$ \textbf{0.83} &  \textbf{61.67} $\pm$ \textbf{0.67} &  \textbf{53.96} $\pm$ \textbf{1.40} &  42.85 $\pm$ 0.79 &  10.77 $\pm$ 0.28 & \textbf{62.34} $\pm$ \textbf{0.67} &  59.63 $\pm$ 1.28 &  49.21 $\pm$ 0.53 &  36.78 $\pm$ 0.50  \\
& NAN & \textbf{64.25} $\pm$ \textbf{0.64} &  56.93 $\pm$ 0.77 &  50.03 $\pm$ 0.62 &  40.45 $\pm$ 0.41 &  \textbf{24.00} $\pm$ \textbf{0.59} & 60.55 $\pm$ 0.71 &  56.40 $\pm$ 1.07 &  52.78 $\pm$ 0.85 &  40.59 $\pm$ 0.84 \\
& Forward & \textbf{64.33} $\pm$ \textbf{0.73} &  47.90 $\pm$ 0.93 &  32.28 $\pm$ 1.10 &  20.00 $\pm$ 0.75 &  7.64 $\pm$ 0.28 & 58.46 $\pm$ 0.53 &  50.82 $\pm$ 0.57 &  43.87 $\pm$ 0.47 &  37.02 $\pm$ 0.72 \\
& Het & \textbf{64.48} $\pm$ \textbf{0.31} &  48.40 $\pm$ 1.32 &  34.26 $\pm$ 0.37 &  20.33 $\pm$ 0.31 &  7.66 $\pm$ 0.38 & 58.18 $\pm$ 0.31 &  51.44 $\pm$ 1.15 &  45.09 $\pm$ 0.40 &  37.43 $\pm$ 0.66 \\
& Het-$\tau$ & \textbf{64.20} $\pm$ \textbf{0.37} &  54.17 $\pm$ 0.79 &  42.03 $\pm$ 0.84 &  22.33 $\pm$ 0.57 &  7.31 $\pm$ 0.37 & \textbf{62.71} $\pm$ \textbf{0.75} &  59.89 $\pm$ 0.54 &  53.75 $\pm$ 1.08 &  41.14 $\pm$ 0.98 \\
& Het-$\tau$-$\bm{\Sigma}_{\textbf{full}}$ & \textbf{65.18} $\pm$ \textbf{0.90} &  54.83 $\pm$ 0.46 &  41.49 $\pm$ 1.53 &  22.42 $\pm$ 0.95 &  7.77 $\pm$ 0.27 & 61.88 $\pm$ 0.85 &  61.29 $\pm$ 0.46 &  56.44 $\pm$ 0.53 &  45.75 $\pm$ 1.02 \\
& LN & \textbf{64.88} $\pm$ \textbf{0.98} &  \textbf{60.58} $\pm$ \textbf{1.07} &  \textbf{55.55} $\pm$ \textbf{1.30} &  \textbf{46.43} $\pm$ \textbf{1.15} &  \textbf{23.64} $\pm$ \textbf{1.02} & \textbf{63.35} $\pm$ \textbf{0.75} &  \textbf{64.31} $\pm$ \textbf{0.98} &  \textbf{64.07} $\pm$ \textbf{0.77} &  \textbf{61.20} $\pm$ \textbf{1.22} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> 7_tables_syntheticnoise_sym.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t!]
\tabcolsep=0.15cm 
\caption{\label{tab:synthetic-sym} \textbf{Synthetic Noise on MNIST, CIFAR-10 and CIFAR-100.} We implement our method and all baselines in the same shared code based and do a search for the best hyperparameters on a noisy validation set for all methods. We report the mean and standard deviation of the test accuracy from five runs with different random seeds. Results in bold correspond to the methods with no statistically significant difference to the method with the highest mean. Our method~(LN) shows strong performance compared to baselines, especially on the  predictable asymmetric noise, and the challenging CIFAR-100 dataset.  
}
\begin{center}
\begin{tabular}{ m{1em} l c c c c c@{}} 
 \toprule
 \multirow{2}{0em}{} & \multirow{2}{4em}{Method} & No Noise & \multicolumn{4}{c}{Symmetric Noise Rate} \\ \cmidrule(lr){3-3}\cmidrule(lr){4-7}
 & & 0\% & 20\% & 40\% & 60\% & 80\% \\
 \midrule
 \multirow{8}{2em}{\rotatebox[origin=c]{90}{MNIST}}
& CE & 99.27 $\pm$ 0.07 &  88.41 $\pm$ 0.34 &  70.67 $\pm$ 1.30 &  51.04 $\pm$ 1.19 &  29.53 $\pm$ 1.08 \\
& GCE & 99.22 $\pm$ 0.06 &  \textbf{98.85} $\pm$ \textbf{0.18} &  \textbf{98.60} $\pm$ \textbf{0.11} &  \textbf{97.45} $\pm$ \textbf{0.31} &  \textbf{92.60} $\pm$ \textbf{0.61} \\
& NAN & 98.44 $\pm$ 0.24 &  97.51 $\pm$ 0.37 &  90.03 $\pm$ 0.95 &  74.00 $\pm$ 2.92 &  46.25 $\pm$ 2.03 \\
& Forward & 99.27 $\pm$ 0.03 &  87.46 $\pm$ 0.70 &  69.96 $\pm$ 2.10 &  50.43 $\pm$ 1.43 &  30.01 $\pm$ 0.60 \\
& Het & 99.28 $\pm$ 0.05 &  87.09 $\pm$ 0.70 &  70.30 $\pm$ 1.10 &  50.57 $\pm$ 1.02 &  29.88 $\pm$ 0.88 \\
& Het-$\tau$ & 99.25 $\pm$ 0.07 &  88.10 $\pm$ 0.70 &  70.19 $\pm$ 1.58 &  51.95 $\pm$ 1.13 &  31.81 $\pm$ 0.86\\
& Het-$\tau$-$\bm{\Sigma}_{\textbf{full}}$ & \textbf{99.25} $\pm$ \textbf{0.15} &  89.16 $\pm$ 0.44 &  70.34 $\pm$ 1.20 &  50.89 $\pm$ 1.79 &  30.54 $\pm$ 0.69 \\
& LN & \textbf{99.38} $\pm$ \textbf{0.06} &  \textbf{98.53} $\pm$ \textbf{0.27} &  97.21 $\pm$ 0.38 &  90.93 $\pm$ 2.29 &  60.15 $\pm$ 5.01 \\
\midrule
\multirow{8}{2em}{\rotatebox[origin=c]{90}{CIFAR-10}} 
& CE & \textbf{90.67} $\pm$ \textbf{0.80} &  73.54 $\pm$ 1.01 &  56.56 $\pm$ 1.44 &  39.44 $\pm$ 1.87 &  21.91 $\pm$ 1.35 \\
& GCE & \textbf{90.83} $\pm$ \textbf{0.44} &  \textbf{87.55} $\pm$ \textbf{0.41} &  \textbf{84.72} $\pm$ \textbf{0.82} &  \textbf{79.25} $\pm$ \textbf{0.93} &  \textbf{64.28} $\pm$ \textbf{1.42} \\
& NAN & 89.61 $\pm$ 0.93 &  83.86 $\pm$ 1.03 &  79.80 $\pm$ 0.59 &  73.58 $\pm$ 0.41 &  61.06 $\pm$ 1.84 \\
& Forward & \textbf{90.69} $\pm$ \textbf{0.38} &  74.39 $\pm$ 1.49 &  59.60 $\pm$ 1.40 &  40.06 $\pm$ 2.16 &  23.80 $\pm$ 1.00 \\
& Het & \textbf{90.41} $\pm$ \textbf{0.69} &  74.67 $\pm$ 1.06 &  58.53 $\pm$ 1.96 &  39.51 $\pm$ 2.53 &  24.18 $\pm$ 0.67 \\
& Het-$\tau$ & \textbf{91.18} $\pm$ \textbf{0.41} &  76.90 $\pm$ 1.79 &  63.55 $\pm$ 2.27 &  44.73 $\pm$ 1.67 &  26.36 $\pm$ 1.58 \\
& Het-$\tau$-$\bm{\Sigma}_{\textbf{full}}$ & \textbf{90.82} $\pm$ \textbf{0.42} &  77.16 $\pm$ 0.94 &  62.85 $\pm$ 1.88 &  44.20 $\pm$ 3.05 &  25.11 $\pm$ 2.20 \\
& LN & 90.17 $\pm$ 0.55 &  86.13 $\pm$ 1.03 &  81.37 $\pm$ 1.97 &  76.08 $\pm$ 0.63 &  \textbf{63.58} $\pm$ \textbf{1.76}\\
\midrule
\multirow{8}{2em}{\rotatebox[origin=c]{90}{CIFAR-100}} 
& CE & \textbf{64.87} $\pm$ \textbf{0.88} &  47.39 $\pm$ 0.43 &  33.62 $\pm$ 0.79 &  20.04 $\pm$ 0.58 &  7.38 $\pm$ 0.12 \\
& GCE & \textbf{64.33} $\pm$ \textbf{0.83} &  \textbf{61.67} $\pm$ \textbf{0.67} &  \textbf{53.96} $\pm$ \textbf{1.40} &  42.85 $\pm$ 0.79 &  10.77 $\pm$ 0.28 \\
& NAN & \textbf{64.25} $\pm$ \textbf{0.64} &  56.93 $\pm$ 0.77 &  50.03 $\pm$ 0.62 &  40.45 $\pm$ 0.41 &  \textbf{24.00} $\pm$ \textbf{0.59} \\
& Forward & \textbf{64.33} $\pm$ \textbf{0.73} &  47.90 $\pm$ 0.93 &  32.28 $\pm$ 1.10 &  20.00 $\pm$ 0.75 &  7.64 $\pm$ 0.28 \\
& Het & \textbf{64.48} $\pm$ \textbf{0.31} &  48.40 $\pm$ 1.32 &  34.26 $\pm$ 0.37 &  20.33 $\pm$ 0.31 &  7.66 $\pm$ 0.38 \\
& Het-$\tau$ & \textbf{64.20} $\pm$ \textbf{0.37} &  54.17 $\pm$ 0.79 &  42.03 $\pm$ 0.84 &  22.33 $\pm$ 0.57 &  7.31 $\pm$ 0.37 \\
& Het-$\tau$-$\bm{\Sigma}_{\textbf{full}}$ & \textbf{65.18} $\pm$ \textbf{0.90} &  54.83 $\pm$ 0.46 &  41.49 $\pm$ 1.53 &  22.42 $\pm$ 0.95 &  7.77 $\pm$ 0.27 \\
& LN & \textbf{64.88} $\pm$ \textbf{0.98} &  \textbf{60.58} $\pm$ \textbf{1.07} &  \textbf{55.55} $\pm$ \textbf{1.30} &  \textbf{46.43} $\pm$ \textbf{1.15} &  \textbf{23.64} $\pm$ \textbf{1.02} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> appendices/histograms_of_mse.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.49\textwidth]{Figures/supplementary/hist_mse-50-bins.pdf}
    \caption{No Caption yet}
    \label{fig:my_label}
\end{figure}
